Stepping OCaml

Steppers, which display all the reduction steps of a given program, are a novice-friendly tool for understanding program behavior. Unfortunately, steppers are not as popular as they ought to be; indeed, the tool is only available in the pedagogical languages of the DrRacket programming environment. We present a stepper for a practical fragment of OCaml. Similarly to the DrRacket stepper, we keep track of evaluation contexts in order to reconstruct the whole program at each reduction step. The difference is that we support effectful constructs, such as exception handling and printing primitives, allowing the stepper to assist a wider range of users. In this paper, we describe the implementation of the stepper, share the feedback from our students, and show an attempt at assessing the educational impact of our stepper.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{P. Achten, H. Miller (Eds.): \\
Trends in Functional Programming in Education 2018 (TFPIE'18)\\
EPTCS 295, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.295.2}{10.4204/EPTCS.295.2}}

